Using Shape to Categorize: Low-Shot Learning with an Explicit Shape Bias

It is widely accepted that reasoning about object shape is important for object recognition. However, the most powerful object recognition methods today do not explicitly make use of object shape during learning. In this work, motivated by recent developments in low-shot learning, findings in developmental psychology, and the increased use of synthetic data in computer vision research, we investigate how reasoning about 3D shape can be used to improve low-shot learning methods' generalization performance. We propose a new way to improve existing low-shot learning approaches by learning a discriminative embedding space using 3D object shape, and using this embedding by learning how to map images into it. Our new approach improves the performance of image-only low-shot learning approaches on multiple datasets. We also introduce Toys4K, a 3D object dataset with the largest number of object categories currently available, which supports low-shot learning.

==> figure_tex/dataset_lowshot_accuracy_fig.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{figure_data/dataset_accuracy.pdf}
\end{center}
\vspace{-10pt}
\caption{Comparison between 1-shot learning performance of SimpleShot on ModelNet40-LS, ShapeNet55-LS and Toys4.3K. The high number of categories in Toys allows for many-way low-shot testing, making low-shot learning on Toys4.3K a challenging task.}
\label{fig:dataset-accuracy}
\end{figure}


==> figure_tex/prelim_setting_fig.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{figure_data/inference_fig.pdf}
\end{center}
\vspace{-10pt}
\caption{Description of how shape and image embeddings are combined by averaging to obtain an object prototype. For the query images no shape information is available, and they are classified based on distance to the object prototypes (mean features).}
\label{fig:setting}
\end{figure}


==> figure_tex/toys45K_dataset_figure.tex <==
\begin{figure*}[h]
\begin{center}
\includegraphics[width=\linewidth]{figure_data/Toys45K_figure_large.png}
\end{center}
\caption{Approximately one third of the objects Toys-4.3K, a new dataset of high quality 3D assets for low-shot object learning using object appearance and shape information.}
\label{fig:toys45K_viz}
\end{figure*}



==> figure_tex/toys45K_stats_figure.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{figure_data/Toys45K_stats.png}
\end{center}
\vspace{-10pt}
\caption{Data distribution for super-ordinate and basic-level categories in Toys4.3K.}
\label{fig:toys45K_distribution}
\end{figure}


==> table_tex/appearance_vs_shape.tex <==
\begin{table}[ht!]
\begin{centering}
\begin{tabular}{c|cc|cc|}
 & \multicolumn{2}{c|}{5-way} & \multicolumn{2}{c|}{10-way}  \\
\hline
& 1-shot & 5-shot &  1-shot & 5-shot \\
\hline
Image       & 58.23 & 73.99 & 45.24 & 62.15 \\    
Point Cloud & 66.02 & 83.61 & 54.44 & 75.26 \\
\hline
\begin{tabular}{@{}c@{}}Img + Ptcld \\ Oracle \end{tabular}   &  68.04 & 82.07 & 57.03 & 73.11
\end{tabular}
\caption{On ModelNet40-LS, low-shot generalization is higher for point-cloud based learning than image based learning, justifying our approach in combining the modalities. Oracle model has access to both image and point cloud information at both training and testing time and results in high generalization performance. See text for details.}
\label{tbl:appearance-vs-shape}
\end{centering}
\end{table}

==> table_tex/dataset_comparison.tex <==
\begin{table}[ht!]
\begin{tabular}{l|c|c|c}
Dataset & \# instances & \# categories & \begin{tabular}{@{}c@{}}surface \vspace{-3pt} \\ appearance\end{tabular}\\
\hline
Toys4.3K   & 4,277     & 108 & PBR  \\    
ModelNet40~\cite{wu20153d} & 12,311    & 40  & N/A \\
ShapeNet~\cite{chang2015shapenet} & ~55,000   & 55  & RGB \\
Thingi10K  & ~10,000   & N/A & N/A \\
ABC        & 750K      & N/A & N/A \\
\hline
\end{tabular}
\caption{Toys4.3K has the most categories of any available dataset of 3D objects. PBR stands for physically based rendering materials, whereas RGB means simple RGB surface color information. Since our work focuses on low-shot learning, the lower total amount of data is not a disadvantage for our dataset.}
\label{tbl:dataset-comparison}
\end{table}

==> table_tex/dataset_statistics.tex <==
\begin{table}[ht!]
\begin{tabular}{l|c|c|c}
Dataset & \# instances & \# categories & \begin{tabular}{@{}c@{}}surface \vspace{-3pt} \\ appearance\end{tabular}\\
\hline
Toys4.3K   & 4,277     & 108 & PBR  \\    
ModelNet40 & 12,311    & 40  & N/A \\
ShapeNet   & ~55,000   & 55  & RGB \\
Thingi10K  & ~10,000   & N/A & N/A \\
ABC        & 750K      & N/A & N/A \\
\hline
\end{tabular}
\caption{Toys4.3K has the most categories of any available dataset of 3D objects. PBR stands for physically based rendering materials, whereas RGB means simple RGB surface color information. Since our work focuses on low-shot learning, the lower total amount of data is not a disadvantage for our dataset.}
\label{tbl:dataset-comparison}
\end{table}
